Optimally Weighted Ensembles of Regression Models: Exact Weight Optimization and Applications

Automated model selection is often proposed to users to choose which machine learning model (or method) to apply to a given regression task. In this paper, we show that combining different regression models can yield better results than selecting a single ('best') regression model, and outline an efficient method that obtains optimally weighted convex linear combination from a heterogeneous set of regression models. More specifically, in this paper, a heuristic weight optimization, used in a preceding conference paper, is replaced by an exact optimization algorithm using convex quadratic programming. We prove convexity of the quadratic programming formulation for the straightforward formulation and for a formulation with weighted data points. The novel weight optimization is not only (more) exact but also more efficient. The methods we develop in this paper are implemented and made available via github-open source. They can be executed on commonly available hardware and offer a transparent and easy to interpret interface. The results indicate that the approach outperforms model selection methods on a range of data sets, including data sets with mixed variable type from drug discovery applications.

==> 06a_QuadraticResults.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/ESTern.pdf}
        \caption{Population and optimal solution found by an heuristic method ((1+1)-Evolutionary Strategy)}
        \label{fig:gull}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/quadProgTern.pdf}
        \caption{Optimal solution found by Quadratic Programming}
        \label{fig:tiger}
    \end{subfigure}
    \caption{All considered individuals are shown as black points, the optimal solution is marked with a white circle and its related RMSE. The Quadratic Programming solution is located close to the optimal solution found by the heuristic method.
    \tb{I might have missed the discussion of this figure in the text ... sorry. Where is it discussed?}}\label{fig:animals}
\end{figure}

==> 07a_WeightedVsUnweighted.tex <==


\begin{table}[!htb]
\begin{tabular}{|l|r|r|r|}
\hline
 Function & y opt & RMSE & weighted RMSE \\ \hline\hline
 ackley-2D & 0 & \textbf{1.8552 (+-~~2.2951)} & 2.1940 (+-~~2.3765~) \\ 
   \hline
ackley-4D & 0 & \textbf{6.0205 (+-~~3.0808)} & 7.9353 (+-~~3.2286~) \\ 
   \hline
GLG-4D-nG80 & 0 & \textbf{20.0680 (+-13.7087)} & 26.2881 (+-~~7.8783~) \\ 
   \hline
GLG-8D-nG320 & 0 & 25.8024 (+-10.0693~) & \textbf{23.8592 (+-10.6014)} \\ 
   \hline
piston & 0 & 0.1648 (+-~~0.0013~) & \textbf{0.1644 (+-~~0.0001)} \\ 
   \hline
robot & 0 & \textbf{0.0060 (+-~~0.0097)} & 0.0087 (+-~~0.0112~) \\ 
   \hline
rosenbrock-4D & 0 & 4.6625 (+-~~1.8603) & \textbf{3.8625 (+-~~2.3275)} \\ 
   \hline
rosenbrock-8D & 0 & 4092.6467 (+-2885.64) & \textbf{3603.4226 (+-1317.70)} \\  % & 4092.6467 (+-2885.6781) & 3603.4226 (+-1317.7002) \\ 
   \hline
shubert-2D & - 186.7309 & \textbf{-148.0154 (+-54.5093)} & -108.1625 (+-58.2592) \\ \hline
  \end{tabular}
  \caption{
  Results achieved on a range of functions, using standard RMSE and RMSE with weighted training points based on density. } 
  %Alles Minimierungsprobleme. Weighted schneidet nicht so gut ab wie erwartet. Fragt sich wieso, weil wir schon das Gegenteil gezeigt hatten. Vielleicht wegen der QuicknDirty Bugfixing Methode?}
\end{table}

==> 11_Glossary.tex <==
\section{Glossary}

\tb{I would not do this; as the variables are all introduced in the paper. It is quite unusual for a conference paper or journal paper to do this.}
List of identifiers specified: \martina{for orientation only, to be commented out later}
\tb{Ah, I see your comment now ...}
\begin{itemize}
    \item $f$ the objective function
    \item $\hat{f}$ the predicted function
    \item $y$ an objective function value
    \item $\hat{y}$ a predicted function value
    \item $x_i$ the set of sample points where the models/functions are evaluated \martina{changed from $t_i$ to $x_i$}
    \item $n$ number of predictions of a single model
    \item $d$ dimension of the search space
    \item $s$ number of surrogate models in the set
    \item $\alpha$ a set of weights for the models in an ensemble, $\alpha_i$ a specific weight for a single model
    \item $k$ number of nearest neighbours considered for density calculation
\end{itemize}

% TODOs:
% \begin{enumerate}
%     \item abstract (ME) {\color{ForestGreen}\Large\textbf{\checkmark}}
%     \item Introduction (ME + MF + alle) {\color{ForestGreen}\Large\textbf{\checkmark}}
%     \item Preliminaries {\color{ForestGreen}\Large\textbf{\checkmark}}
%     \item Related Work (ME)
%     \item Local Density Weighted Cross-Validation (MF) {\color{ForestGreen}\Large\textbf{\checkmark}}
%     \item n-ary Ensembles (MF) {\color{ForestGreen}\Large\textbf{\checkmark}}
%     \item Exact Quadratic Programming Method (JB)
%     \item Comparison of approaches (PE)
%     \item Results and Discussion (alle)
%     \item summary and outlook (alle)
% \end{enumerate}

==> delete_PreviousIdeas.tex <==


\used{Dissertation}{
%
%{\color{kommentar}**************************************************}

\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{\textwidth} 
    	\caption{One base model always predicts a smaller value than the other}   
        \label{fig:2predicitons:a}
		\includegraphics[width=\textwidth]{figures/2predictionsParallel.pdf}    	
    \end{subfigure}
 	\begin{subfigure}[b]{\textwidth} 
    	\caption{Each model predicts larger in one and smaller in the other case}
        \label{fig:2predicitons:b}
		\includegraphics[width=\textwidth]{figures/2predictionsOpposing.pdf}    	
    \end{subfigure}
    \caption{Both plots show a set of combinations of two predictions made by two base models (red and blue) along with the resulting predictions made generated through convex linear combining using a fixed step width of $0.1$. The second row of each plot displays the related RMSE values resulting from the combination of the two predictions.}
    \label{fig:2predicitons}
\end{figure}
However, when evaluating the ensemble built by the proposed method of building convex linear combinations, this is not done based on a single prediction but on a set of predictions. Also, calculating the RMSE of a single prediction only yields the simple prediction error. Questions that also have to be considered are:
\begin{itemize}
    \item Do these findings made for single predictions still apply for multiple predictions?
    \item How does the RMSE influence the evaluation of the models' overall performance?
\end{itemize}

To answer these additional questions, the analysis is extended to two predictions.
Figure \ref{fig:2predicitons} displays several possible combinations of predictions for such a setup. Figure~\ref{fig:2predicitons:a} shows a set of predictions where the one model always predicts a larger value than the other model, while in Figure~\ref{fig:2predicitons:b} one model always returns a larger prediction for one point and a smaller prediction for the other point. In both plots, like before, the upper row shows the predictions, base model predictions are colored blue or red, and predictions of the linear combinations are colored white. The lower row displays the relating RMSE values resulting from the two predictions.

We can see from these plots, that it does not suffice for the ensemble prediction to be better than the base models, when in one of the two cases the prediction spans the actual function value, while the combined predictions of one of the base models are better in terms of RMSE (cf. Fig. \ref{fig:2predicitons:a} items 2-5, \ref{fig:2predicitons:b} items 6-7). The combined prediction error, in terms of RMSE, rather benefits from opposing errors in general (cf. \ref{fig:2predicitons:a} items 6-9, \ref{fig:2predicitons:b} items 1-5).

As mentioned before, the CCM can make a better prediction on a single point only if the predictions of the base models span the true function value.\\ 
However, regarding more than one prediction, this evaluation is influenced by the characteristics of the RMSE. The overall fit of the CCM, in terms of RMSE, can be better than both base models also, when none of the base models predictions is spanning the true function value. For such an evaluation it is sufficient when one model returns a larger prediction than the other model for one point, and a smaller prediction for the other point.

Noticeable is also, that in contrast to the plots shown in Figure~\ref{fig:1prediciton}, the points marking the RMSE values in most of the cases lie on a parabolic curve. This might indicate that the search space, generated by the RMSE could also be convex. Interpreting the RMSE as a function describing a form of mean squared distance would support this claim. However, this assumption is based on observations only and would require further analysis.}

==> delete_Problem.tex <==
\section{Problem}\label{problem_section}




\plan{main question}\\
If the fitness function used to find the optimal weights of the ensemble is convex a more efficient search / gradient based could be applied. Or the optimal point might even be calculated. \bn{To be put to the Introduction? Can also be repeated here.}
\\





==> delete_Proof.tex <==
\section{Dimension 1 - two models}
\subsection{Single Prediction}
We consider two base models and their related convex combinations of models (CCMs) making a single prediction. For reasons of simplicity and without loss of generality, we assume, that the real function value is zero and that the base models are making different prediction errors.
\begin{figure}[h!tb]
	\centering
	\includegraphics[width=\textwidth]{figures/1prediction.pdf}
    \caption{\used{thesis}{The upper row plots show the predictions of two base models and its related CCMs for a single point. The true function value of zero is marked with a line. In the lower row the related RMSEs are given. The best prediction and the related smallest prediction error are marked with an additional circle. It can be seen that in some cases the CCM performs better than both base models, but it never performs worse than both.}}
    \label{fig:1prediciton}
\end{figure}

\used{thesis}{Figure \ref{fig:1prediciton} displays such a situation.  In the upper row, the colored points mark the predictions of the base models, while the white points mark the predictions obtained through convex linear combination. The true function value is set to zero, displayed by the horizontal line.\\ 
The lower row depicts the related resulting RMSEs.\\
All other possible relations between prediction errors and resulting RMSE can be easily derived from this. So would a change of the distance between the base models predictions result in a steepened slope, while a larger distance between the two predictions and the real function value would result in a larger absolute error. 
}\\
Since we are only considering a single prediction, the resulting RMSE equals the single absolute prediction error.
\[RMSE_{n=1}=\sqrt{\frac{1}{1}\sum_{i=1}^{1}{(y_1-\hat{y}_1)^2}}=\sqrt{(y-\hat{y})^2}=|y-\hat{y}|=AE\]
The resulting fitness function in this case is a linear function that is strictly monotonically decreasing for $\alpha$-values smaller than the optimal $\alpha$-value and strictly monotonically increasing for $\alpha$-values larger than the optimal $\alpha$-value.

Therefore, the fitness is a piecewise linear, convex function. 

\subsection{Two Predictions}
Specify RMSE as fitness function of $\alpha$ and determine first+second derivative???\\

The CCM was previously defined as a weighted sum using a number of weights according to the number of models used. Due to the convex definition of the combination to $n-1$ weights in the case of $n$ models. Therefore, in the following the value $\alpha$ is used to represent the values $\alpha_1=\alpha$ and $\alpha_2=1-\alpha$. Using this specification the CCM can be given as: $\sum_{i=1}^s \alpha_i \hat{y}_i = \alpha\hat{y_1} + (1-\alpha)\hat{y_2}$.\\

The fitness function specified by the RMSE can then be given as a function of $\alpha$ as:
\[
RMSE(\alpha)=\sqrt{\frac{1}{n}\sum_{i=1}^{n}{(y_i-(\alpha\hat{y_1} + (1-\alpha)\hat{y_2}))^2}}
\]

~\\~ \vspace{2em} ~\\
\idea{Or: The sum of two convex functions is also convex. This may be a better approach}

The error function, resulting from two models for one prediction is a linear, and therefore convex, function of alpha:
\[E(\alpha)= y - \left(\alpha\hat{y_1} + (1-\alpha)\hat{y_2}\right)\]

The square of a convex function remains convex, thus the square of the error function $SE$ is also convex:
\[SE(\alpha)= y - \left(\alpha\hat{y_1} + (1-\alpha)\hat{y_2}\right)^2\]

The sum of two convex functions preserves the convexity. What about the mean and the root?


\begin{figure}[h!tbp]
	\centering
	\begin{subfigure}[b]{\textwidth} 
    	\caption{One base model always predicts a smaller value than the other}   
        \label{fig:2predicitons:a}
		\includegraphics[width=\textwidth]{figures/2predictionsParallel.pdf}    	
    \end{subfigure}
 	\begin{subfigure}[b]{\textwidth} 
    	\caption{Each model predicts larger in one and smaller in the other case}
        \label{fig:2predicitons:b}
		\includegraphics[width=\textwidth]{figures/2predictionsOpposing.pdf}    	
    \end{subfigure}
    \caption{\used{thesis}{Both plots show a set of combinations of two predictions made by two base models (red and blue) along with the resulting predictions made generated through convex linear combining using a fixed step width of $0.1$. The second row of each plot displays the related RMSE values resulting from the combination of the two predictions.}}
    \label{fig:2predicitons}
\end{figure}

\section{Step from Dimension n to n-1}
Every mixture of two models can be fixed for an arbitrary weight. This way the dimension of the problem can be reduced by one.

